DiffusionPhase: Motion Diffusion in Frequency Domain

In this study, we introduce a learning-based method for generating high-quality human motion sequences from text descriptions (e.g., ``A person walks forward"). Existing techniques struggle with motion diversity and smooth transitions in generating arbitrary-length motion sequences, due to limited text-to-motion datasets and the pose representations used that often lack expressiveness or compactness. To address these issues, we propose the first method for text-conditioned human motion generation in the frequency domain of motions. We develop a network encoder that converts the motion space into a compact yet expressive parameterized phase space with high-frequency details encoded, capturing the local periodicity of motions in time and space with high accuracy. We also introduce a conditional diffusion model for predicting periodic motion parameters based on text descriptions and a start pose, efficiently achieving smooth transitions between motion sequences associated with different text descriptions. Experiments demonstrate that our approach outperforms current methods in generating a broader variety of high-quality motions, and synthesizing long sequences with natural transitions.

==> sec/tables/Humanml_results.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|lllll|}
\hline
%extend this source page to full-right for filling in numbers
\multicolumn{1}{|l|}{Length}                                                    & Method            & Top-3 R-Precision ↑ & FID ↓ & MM-DIST ↓ & Diversity → & MModality ↑            \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}Default \\ Length\end{tabular}}      & Real              & \multicolumn{1}{c}{0.797}               & \multicolumn{1}{c}{0.002} & \multicolumn{1}{c}{2.974}     & \multicolumn{1}{c}{9.503}       & \multicolumn{1}{c|}{-} \\ \cline{2-7}
                                                                                & Language2Pose     & \multicolumn{1}{c}{0.486}               & \multicolumn{1}{c}{11.02} & \multicolumn{1}{c}{5.296}     & \multicolumn{1}{c}{7.676}       & \multicolumn{1}{c|}{-} \\
                                                                                & Text2Gestures      & \multicolumn{1}{c}{0.345}               & \multicolumn{1}{c}{5.012} & \multicolumn{1}{c}{6.030}     & \multicolumn{1}{c}{6.409}       & \multicolumn{1}{c|}{-}\\
                                                                                & Dance2Music       & \multicolumn{1}{c}{0.097}               & \multicolumn{1}{c}{66.98} & \multicolumn{1}{c}{8.116}     & \multicolumn{1}{c}{0.725}       & \multicolumn{1}{c|}{0.043} \\
                                                                                & MOCOGAN           & \multicolumn{1}{c}{0.106}               & \multicolumn{1}{c}{94.41} & \multicolumn{1}{c}{9.643}     & \multicolumn{1}{c}{0.462}       & \multicolumn{1}{c|}{0.019}                \\ % This is the new row
                                                                                & Guo et al.        & \multicolumn{1}{c}{0.736}               & \multicolumn{1}{c}{1.087} & \multicolumn{1}{c}{3.347}     & \multicolumn{1}{c}{9.175}       & \multicolumn{1}{c|}{2.219}                 \\
                                                                                & MDM               & \multicolumn{1}{c}{0.611}               & \multicolumn{1}{c}{0.544} & \multicolumn{1}{c}{5.566}     & \multicolumn{1}{c}{\colorbox{red}{9.559}}       & \multicolumn{1}{c|}{\colorbox{orange}{2.799}}                 \\
                                                                                & MotionDiffuse     & \multicolumn{1}{c}{\colorbox{red}{0.782}}               & \multicolumn{1}{c}{0.630} & \multicolumn{1}{c}{\colorbox{red}{3.113}}     & \multicolumn{1}{c}{\colorbox{orange}{9.410}}       & \multicolumn{1}{c|}{1.553}                 \\ 
                                                                                & T2M     & \multicolumn{1}{c}{\colorbox{orange}{0.775}}               & \multicolumn{1}{c}{\colorbox{red}{0.141}} & \multicolumn{1}{c}{\colorbox{orange}{3.121}}     & \multicolumn{1}{c}{9.722}       & \multicolumn{1}{c|}{1.831} \\  
                                                                                & MLD     & \multicolumn{1}{c}{\colorbox{yellow}{0.772}}               & \multicolumn{1}{c}{\colorbox{yellow}{0.473}} & \multicolumn{1}{c}{3.196}     & \multicolumn{1}{c}{9.724}       & \multicolumn{1}{c|}{\colorbox{yellow}{2.413}}  \\
                                                                                \cline{2-7} 
                                                                                & Ours              &     \multicolumn{1}{c}{0.761}     &   \multicolumn{1}{c}{\colorbox{orange}{0.397}}    &    \multicolumn{1}{c}{\colorbox{yellow}{3.194}}       &  \multicolumn{1}{c}{\colorbox{yellow}{9.363}}             &      \multicolumn{1}{c|}{\colorbox{red}{2.805}}                   \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}3x\\ Default\\ Length\end{tabular}} & Guo et al.        &   \multicolumn{1}{c}{0.496}   &   \multicolumn{1}{c}{8.701}    &     \multicolumn{1}{c}{\colorbox{yellow}{4.947}}       &       \multicolumn{1}{c}{7.370}      &        \multicolumn{1}{c|}{-}             \\
                                                                                & MDM               &      \multicolumn{1}{c}{0.121}    &   \multicolumn{1}{c}{18.499}  &    \multicolumn{1}{c}{9.706}        &    \multicolumn{1}{c}{5.806}          &      \multicolumn{1}{c|}{-}                 \\
                                                                                & MotionDiffuse     &     \multicolumn{1}{c}{0.392}   &  \multicolumn{1}{c}{10.303}     &      \multicolumn{1}{c}{5.819}     &   \multicolumn{1}{c}{5.928}          &            \multicolumn{1}{c|}{-}             \\ 
                                                                                 & MLD     & \multicolumn{1}{c}{\colorbox{yellow}{0.546}}               & \multicolumn{1}{c}{\colorbox{yellow}{7.842}} & \multicolumn{1}{c}{4.976}     & \multicolumn{1}{c}{\colorbox{yellow}{7.938}}       & \multicolumn{1}{c|}{-} \\
                                                                                \cline{2-7} 
                                                                                & Ours (Repetition) &     \multicolumn{1}{c}{\colorbox{red}{0.751}}      &   \multicolumn{1}{c}{\colorbox{red}{0.385}}     &    \multicolumn{1}{c}{\colorbox{red}{3.266}}       &   \multicolumn{1}{c}{\colorbox{red}{9.009}}          &         \multicolumn{1}{c|}{2.802}               \\
                                                                                & Ours (Generative) &   \multicolumn{1}{c}{\colorbox{orange}{0.725}}   &  \multicolumn{1}{c}{\colorbox{orange}{0.584}}      &   \multicolumn{1}{c}{\colorbox{orange}{3.311}}  &    \multicolumn{1}{c}{\colorbox{orange}{8.884}}  & \multicolumn{1}{c|}{2.817}                     \\ \hline
\end{tabular}
}
\caption{Results for HumanML3D test set. The best, second-best, and third-best results are highlighted in red, orange, and yellow, respectively. Our method achieves comparable results to the baseline methods in the Default Length setting and significantly better results in the $3\times$ Default Length.}
\label{tab:humanml results}
\vspace{-.5cm}
\end{table}


==> sec/tables/KIT_results.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|l|lllll|}
\hline
%extend this source page to full-right for filling in numbers
\multicolumn{1}{|l|}{Length}                                                    & Method            & Top-3 R-Precision ↑ & FID ↓ & MM-DIST ↓ & Diversity → & MModality ↑            \\ \hline
\multirow{10}{*}{\begin{tabular}[c]{@{}c@{}}Default \\ Length\end{tabular}}    & Real              & \multicolumn{1}{c}{0.779}               & \multicolumn{1}{c}{0.031} & \multicolumn{1}{c}{2.788}     & \multicolumn{1}{c}{11.08}       & \multicolumn{1}{c|}{-} \\ \cline{2-7} 
                                                                                & Language2Pose     & \multicolumn{1}{c}{0.483}               & \multicolumn{1}{c}{6.545} & \multicolumn{1}{c}{5.147}     & \multicolumn{1}{c}{9.073}       & \multicolumn{1}{c|}{-} \\
                                                                                & Text2Gestures      & \multicolumn{1}{c}{0.338}               & \multicolumn{1}{c}{12.12} & \multicolumn{1}{c}{6.964}     & \multicolumn{1}{c}{9.334}       & \multicolumn{1}{c|}{-} \\
                                                                                & Dance2Music       & \multicolumn{1}{c}{0.086}               & \multicolumn{1}{c}{115.4} & \multicolumn{1}{c}{10.40}     & \multicolumn{1}{c}{0.241}       & \multicolumn{1}{c|}{0.062} \\
                                                                                & MOCOGAN           & \multicolumn{1}{c}{0.063}               & \multicolumn{1}{c}{82.69} & \multicolumn{1}{c}{10.47}     & \multicolumn{1}{c}{3.091}       & \multicolumn{1}{c|}{0.250} \\ % This is the new row
                                                                                & Guo et al.        & \multicolumn{1}{c}{0.681}               & \multicolumn{1}{c}{3.022} & \multicolumn{1}{c}{3.488}     & \multicolumn{1}{c}{10.720}       & \multicolumn{1}{c|}{\colorbox{yellow}{2.052}}                 \\
                                                                                & MDM               & \multicolumn{1}{c}{0.396}               & \multicolumn{1}{c}{\colorbox{orange}{0.497}} & \multicolumn{1}{c}{9.191}     & \multicolumn{1}{c}{10.847}      & \multicolumn{1}{c|}{1.907}                       \\
                                                                                & MotionDiffuse     & \multicolumn{1}{c}{\colorbox{orange}{0.739}}               & \multicolumn{1}{c}{1.954} & \multicolumn{1}{c}{\colorbox{red}{2.958}}     & \multicolumn{1}{c}{\colorbox{red}{11.100}}       & \multicolumn{1}{c|}{0.730}                       \\ 
                                                                                & T2M               & \multicolumn{1}{c}{\colorbox{red}{0.745} }              & \multicolumn{1}{c}{0.514} & \multicolumn{1}{c}{\colorbox{orange}{3.007}}     & \multicolumn{1}{c}{\colorbox{orange}{10.921}}      & \multicolumn{1}{c|}{1.570}                       \\
                                                                                & MLD               & \multicolumn{1}{c}{0.734}               & \multicolumn{1}{c}{\colorbox{red}{0.404}} & \multicolumn{1}{c}{3.204}     & \multicolumn{1}{c}{10.800}      & \multicolumn{1}{c|}{\colorbox{red}{2.192}}                       \\
                                                                                \cline{2-7} 
                                                                                & Ours              &     \multicolumn{1}{c}{\colorbox{yellow}{0.736}}          &  \multicolumn{1}{c}{\colorbox{yellow}{0.503}}     &   \multicolumn{1}{c}{\colorbox{yellow}{3.167}}        &      \multicolumn{1}{c}{\colorbox{yellow}{10.873}}       &        \multicolumn{1}{c|}{\colorbox{orange}{2.071}}                \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}3x\\ Default\\ Length\end{tabular}} & Guo et al.        &     \multicolumn{1}{c}{\colorbox{yellow}{0.551}}                 &  \multicolumn{1}{c}{\colorbox{yellow}{7.591}}       &    \multicolumn{1}{c}{\colorbox{yellow}{4.907}}        &     \multicolumn{1}{c}{\colorbox{yellow}{8.767}}        &      \multicolumn{1}{c|}{-}                  \\
                                                                                & MDM     &      \multicolumn{1}{c}{0.094}               &   \multicolumn{1}{c}{41.760}       &      \multicolumn{1}{c}{11.228}       &   \multicolumn{1}{c}{5.588}          &    \multicolumn{1}{c|}{-}                                   \\           
                                                                                
                                                                                & MotionDiffuse      &          \multicolumn{1}{c}{0.281}             &     \multicolumn{1}{c}{72.225}     &   \multicolumn{1}{c}{9.961}         &      \multicolumn{1}{c}{6.119}       &         \multicolumn{1}{c|}{-}                
                                                                                
                                                                                \\\cline{2-7} 
                                                                                & Ours (Repetition) &   \multicolumn{1}{c}{\colorbox{red}{0.727}}        &    \multicolumn{1}{c}{\colorbox{red}{0.902}}   &   \multicolumn{1}{c}{\colorbox{orange}{3.429}}  & \multicolumn{1}{c}{\colorbox{red}{10.067}}   &     \multicolumn{1}{c|}{1.968}  \\
                                                                                & Ours (Generative) &     \multicolumn{1}{c}{\colorbox{orange}{0.710}}                &   \multicolumn{1}{c}{\colorbox{orange}{1.174}}    &      \multicolumn{1}{c}{\colorbox{red}{3.483}}     &      \multicolumn{1}{c}{\colorbox{orange}{9.813}}        &               \multicolumn{1}{c|}{2.196}         \\ \hline
\end{tabular}
}
\caption{Results for KIT-ML test set. The best, second-best, and third-best results are highlighted in red, orange, and yellow, respectively.}
\label{tab:KIT results}
\vspace{-0.2cm}
\end{table}


==> sec/tables/ablation.tex <==
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{|c|ccc|ccc|}
\hline
                         & \multicolumn{3}{c|}{Setting}                                              & \multicolumn{3}{c|}{Metrics}                                                               \\ \cline{2-7} 
\multirow{-2}{*}{Method} & \multicolumn{1}{l}{Highest Freq} & Representation & Num of Phases         & Top-1                        & Top-3                        & FID                          \\ \hline
                         & 8                                & sin            & 128                   & {\color[HTML]{000000} 0.457} & {\color[HTML]{000000} 0.784} & {\color[HTML]{000000} 0.232} \\
                         & 30                               & sin            & 128                   & \multicolumn{1}{l}{0.499}    & \multicolumn{1}{l}{0.789}    & \multicolumn{1}{l|}{0.106}   \\
                         & 30                               & sin, cos       & 128                   & \colorbox{orange}{0.506}                        & \colorbox{orange}{0.791}                        & \colorbox{orange}{0.082}                        \\
\multirow{-4}{*}{Ours}   & 30                               & sin, cos       & 256                   & \colorbox{red}{0.507}                        & \colorbox{red}{0.792}                        & \colorbox{red}{0.080}                        \\ \hline
DeepPhase                & -                                & sin            & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}         & \multicolumn{1}{l|}{}        \\ \hline
\end{tabular}
\caption{Reconstruction results of using different settings of phases. The best and second-best results are highlighted in red and orange, respectively. We set our configuration to the highest frequency of $30$, using both sine and cosine representations, with a total of 256 phases, because improvement gained from setting the number of phases to 256 is marginal, and using more phases may also lead to a decline in computational speed.}
\label{ablation}
\end{table}
